Deep Projective Rotation Estimation through Relative Supervision

Orientation estimation is the core to a variety of vision and robotics tasks such as camera and object pose estimation. Deep learning has offered a way to develop image-based orientation estimators; however, such estimators often require training on a large labeled dataset, which can be time-intensive to collect. In this work, we explore whether self-supervised learning from unlabeled data can be used to alleviate this issue. Specifically, we assume access to estimates of the relative orientation between neighboring poses, such that can be obtained via a local alignment method. While self-supervised learning has been used successfully for translational object keypoints, in this work, we show that naively applying relative supervision to the rotational group $SO(3)$ will often fail to converge due to the non-convexity of the rotational space. To tackle this challenge, we propose a new algorithm for self-supervised orientation estimation which utilizes Modified Rodrigues Parameters to stereographically project the closed manifold of $SO(3)$ to the open manifold of $\mathbb{R}^{3}$, allowing the optimization to be done in an open Euclidean space. We empirically validate the benefits of the proposed algorithm for rotational averaging problem in two settings: (1) direct optimization on rotation parameters, and (2) optimization of parameters of a convolutional neural network that predicts object orientations from images. In both settings, we demonstrate that our proposed algorithm is able to converge to a consistent relative orientation frame much faster than algorithms that purely operate in the $SO(3)$ space. Additional information can be found at https://sites.google.com/view/deep-projective-rotation/home .

==> figures/direct_convergence_50_200.tex <==
\begin{figure}[t]
 	\centering
%  	\includegraphics[width=0.7\columnwidth]{figures/N50_S200/mrp_N50_200.png}
%  	\includegraphics[width=0.7\columnwidth]{figures/N50_S200/SO3_N50_200.png}
%  	\includegraphics[width=0.7\columnwidth]{figures/N50_S200/pgm_N50_200.png}
%  	\includegraphics[width=0.7\columnwidth]{figures/N50_S200/quat_N50_200.png}
%  	 \includegraphics[width=0.7\columnwidth]{figures/N50_S200/mrpgradient_N50_200.png}
 	 \includegraphics[width=\columnwidth]{figures/error_N50_S200.pdf}
%  	\vspace{-1em}
 	\caption{Relative Rotation Consensus with Direct Parameter Optimization over 50 orientations. Mean geodesic error between all pairs of rotations after 30k optimization steps. }
 	\label{fig:direct_convergence_50_200}
\end{figure}

==> figures/direct_convergence_50_50.tex <==
\begin{figure}[t]
 	\centering
 	\includegraphics[width=0.7\columnwidth]{figures/N50_S50/mrp_N50_S50.png} 
 	\includegraphics[width=0.7\columnwidth]{figures/N50_S50/SO3_N50_S50.png}
 	\includegraphics[width=0.7\columnwidth]{figures/N50_S50/pgm_N50_S50.png}
 	\includegraphics[width=0.7\columnwidth]{figures/N50_S50/quat_N50_S50.png} 
  	\includegraphics[width=0.7\columnwidth]{figures/N50_S50/mrpgradient_N50_S50.png}
 
%  	\vspace{-1em}
 	\caption{Relative Rotation Consensus with Direct Parameter Optimization. Mean geodesic error between all pairs of rotations after 150k optimization steps. }
 	\label{fig:direct_convergence_50_50}
\end{figure}

==> figures/nn_qualitative.tex <==
\begin{figure}[t]
 	\centering
 	\includegraphics[width=\columnwidth,trim={290 110 150 200},clip]{figures/drill_qualitative.pdf}
%  	\vspace{-1em}
 	\caption{Estimated rotation frame learned for the YCB~\cite{xiang2018posecnn} drill model using Iterative Modified Rodrigues Projective Averaging and relative rotations. The learned X axis is in \textcolor{red}{red}, the Y axis is in \textcolor{green}{green}, and the Z axis is in \textcolor{blue}{blue}.}
 	\label{fig:nn_qualitative}
\end{figure}

==> figures/pascal_sofa_bike.tex <==
\begin{figure}[t]
 	\centering
 
 	\begin{subfigure}{0.45\textwidth}
        \centering
     	\includegraphics[width=\textwidth, trim={0 0 0 0},clip]{figures/pascal_sofa_8runs.png}
 
 	\end{subfigure}
    \begin{subfigure}{0.45\textwidth}
        \centering
     	\includegraphics[width=\textwidth]{figures/pascal_bicycle_8runs.png}
 
    \end{subfigure}
 
 	\caption{\rebuttal{Relative rotation consensus with direct optimization of rotation parameters over 50 unique environments with 100 random generated orientations each (\textbf{left})} and Alamo 1DSfM~\cite{wilson_eccv2014_1dsfm} (\textbf{right}).
 	 Median average-pair-wise angular error (${}^\circ$) between each estimated rotations is shown, with shaded region representing the first and third quartile for each method. The max average-pair-wise angular error for each algorithm at each iteration is shown as a dashed line.
 	 } 
 
 	\label{fig:pascal_sofa_bike}
\end{figure}

==> figures/supervised_mrp.tex <==
\begin{figure}[H]
 	\centering
     	\includegraphics[width=0.7\textwidth]{figures/supervised_orientation.png}
 	\caption{\rebuttal{\textbf{Comparison of Object Orientation Estimation Performance from 2D Images using Absolute Supervision between Quaternions and MRP Parameterization.}
 	        Mean global train pairwise angular error (${}^\circ$) over a set of 100 images of YCB drill rendered at random orientations throughout training iteraions is showed in solid line for each rotation parameterization. Trained for 10K training steps over 8 different seeds per method. Median average-pairwise angular error (${}^\circ$) is shown with shaded areas representing the first and third quartile over all training sessions. The max average-pairwise angular error for each algorithm at each iteration is shown as a dashed line.}
 	 }
 
\label{fig:supervised_orientation}
 	 
\end{figure}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}

==> tables/ablation_fewshot.tex <==
% \begin{table}[ht]
% \begin{varwidth}[b]{0.1\linewidth}
%     \centering
%       \renewcommand{\arraystretch}{1}
%     %  \resizebox{6\linewidth}{!}{
%     \begin{tabular}{c|c c c}
%     % \hline
%     \textbf{Model} & \multicolumn{3}{c} \#\textbf{Demos Used }\\
%     \hline
%           & 1 & 5 & 10\\
%          \hline
%          DON \cite{florence2018dense}  & 0.32 &0.36 & 0.45\\
%          NDF \cite{simeonov2021neural} &  0.46 & 0.70 & 0.88 \\
%           TAX-Pose (Ours) & \textbf{0.77}& \textbf{0.90}& \textbf{0.96}\\
         
%     \hline
%     \end{tabular}
%  % }
%     \caption{Analysis of Number of Demonstrations Used in Training on Upright Pose Mug Hanging Task Success}
%      \label{tab:mug_on_rack_few_shot}
% \end{varwidth}%
% \qquad
% \begin{varwidth}[b]{}
%     \centering
%       
%      
%     \begin{tabular}{c|c c c}
%     \hline
%     \textbf{Ablation} & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
%          \hline
%          No Residual Correspondence  & 0.97 &0.96 & 0.93\\
%          Unweighted SVD &  0.92 & 0.94 & 0.88 \\
%          3-Layer MLP In Place of Attention &  0.90 & 0.82 & 0.76 \\
%          TAX-Pose (Ours)  & \textbf{0.99}& \textbf{0.97}& \textbf{0.96}\\
%     \hline
%     \end{tabular}
%      
%     \caption{Mug Hanging Ablations Results}
%     \label{tab:mug_rack_ablation}
% \end{varwidth}%



% \end{table}


% \begin{table}[htb]
    \noindent \begin{minipage}[t]{.4\textwidth}
    \label{tab:mug_on_rack_few_shot}
    % \small
        \centering
        \begin{tabular}{c|c c c}
            \hline
            \textbf{Model} & \multicolumn{3}{c} \#\textbf{Demos Used }\\
            \hline
            & 1 & 5 & 10\\
            \hline
            DON \cite{florence2018dense}  & 0.32 &0.36 & 0.45\\
            NDF \cite{simeonov2021neural} &  0.46 & 0.70 & 0.88 \\
            \textbf{TAX-Pose (Ours)} & \textbf{0.77}& \textbf{0.90}& \textbf{0.96}\\
            \hline
        \end{tabular}
        \captionof{table}{ \# Demos vs. Overall Success}

    \end{minipage}%
    \qquad\qquad
    \begin{minipage}[t]{.5\textwidth}
        % \small
        \centering
        \label{tab:mug_rack_ablation}
        \begin{tabular}{c|c c c}
            \hline
            \textbf{Ablation} & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
            \hline
            No Res. Corresp.  & 0.97 &0.96 & 0.93\\
            Unweighted SVD &  0.92 & 0.94 & 0.88 \\
            %  3-Layer MLP In Place of Attention &  0.90 & 0.82 & 0.76 \\
            No Attention &  0.90 & 0.82 & 0.76 \\
            \textbf{TAX-Pose (Ours)} & \textbf{0.99}& \textbf{0.97}& \textbf{0.96}\\
            \hline
        \end{tabular}
        \captionof{table}{Mug Hanging Ablations Results}

    \end{minipage}%
% \end{table}


==> tables/direct_mean_median.tex <==
\begin{table}[b]
    \centering
    \begin{tabular}{c|c c c}
    \hline
    Algorithm & Mean Error (${}^{\circ}$) & Median Error (${}^{\circ}$) & $5^{\circ}$ Acc (\%)\\
    \hline
    $SO(3)$  & 2.06 & 0.102 & 96 \\
     $SO(3)$ w/ PMG~\cite{chen2021projective} &  1.97 &0.14 & 92 \\
     Quaternion & 9.72 & 0.04 & 82\\
     MRP (Ours) & \textbf{0.004} & \textbf{0.004} & \textbf{100}\\
     
    \hline
    \end{tabular}
    \caption{Final mean and median average-pair-wise angular error (${}^{\circ}$), percentage of experiments achieving $5^{\circ}$ accuracy after 300K optimization steps over 50 unique environments with 100 randomly generated orientations each.}
    %in $SO(3)$.} 
    % each. , run over 50 sets of orientation sets each with 100 randomly generated orientations in $SO(3)$}
    \label{tab:direct_mean_median}
\end{table}

==> tables/exec-l2-dist-merged.tex <==
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{|lr|rl|ll|ll|ll|ll|ll|ll|ll|ll|ll|}
\hline
\rule{0pt}{2.5em}
 & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} & \multicolumn{2}{c|}{\clipart{chair}} & \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{fridge}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{washingmachine}} & \multicolumn{2}{c|}{\clipart{safe}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-22} 
 & \multicolumn{1}{l|}{} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Baselines}}} & E2E BC & 0.70 & 0.80 & 0.83 & 0.90 & 0.70 & 0.92 & 0.70 & 0.86 & 0.73 & 0.74 & 0.66 & 0.87 & 0.74 & 0.69 & 0.63 & 0.67 & 0.63 & 0.75 & 0.72 & 0.83 \\
\multicolumn{1}{|l|}{} & E2E DAgger & 0.57 & 0.70 & 0.79 & 0.82 & 0.66 & 0.65 & 0.63 & 0.62 & 0.49 & 0.66 & 0.64 & 0.67 & 0.50 & 0.85 & 0.54 & 0.75 & 0.43 & 0.70 & 0.45 & 0.61 \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Ablations}}} & Traj. Flow & 0.26 & 0.50 & 0.46 & 0.50 & 0.16 & 0.38 & 0.19 & 0.48 & 0.30 & 0.50 & 0.13 & 0.55 & 0.28 & 0.57 & 0.44 & 0.50 & 0.14 & 0.63 & 0.24 & 0.40 \\
\multicolumn{1}{|l|}{} & Goal Flow & 0.14 & 0.68 & 0.16 & 0.69 & 0.10 & 0.73 & 0.10 & 0.84 & 0.17 & 0.76 & \textbf{0.05} & 0.88 & 0.12 & 0.51 & 0.29 & 0.54 & 0.12 & 0.68 & 0.16 & 0.47 \\ \hline
\multicolumn{1}{|l|}{\textbf{Ours}} & \textbf{ACRONYM} & \textbf{0.11} & \textbf{0.10} &\textbf{ 0.12 }& \textbf{0.09} & \textbf{0.02} & \textbf{0.04} & \textbf{0.06} & \textbf{0.08} & \textbf{0.15} & \textbf{0.11} & 0.05 & \textbf{0.05} & \textbf{0.12} & \textbf{0.08} & \textbf{0.28} & \textbf{0.26} & \textbf{0.10 }& \textbf{0.09} & \textbf{0.07} & \textbf{0.06} \\ \hline
\end{tabular}
}
\caption{Execution Normalized L2 Distance Metric Results ($\downarrow$): Normalized L2 distances to the ground truth goal position after rollouts. The lower the better.}
\label{tab:exec-l2-dist}
\end{table*}

==> tables/exec-l2-dist.tex <==
\begin{table*}[ht]
\renewcommand{\arraystretch}{1.2}
% \resizebox{\textwidth}{!}{
\centering
\resizebox{0.6\textwidth}{!}{
\setlength\tabcolsep{.2em}
\begin{tabular}{|r|c|ccccccccc|}
 \hline
 \rule{0pt}{2.5em}
 & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} & \multicolumn{2}{c|}{\clipart{chair}} & \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{fridge}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{washingmachine}} & \multicolumn{2}{c|}{\clipart{safe}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-22} 
 & \multicolumn{1}{l|}{} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} \\
\hline
 \textbf{Baselines} & \multicolumn{10}{c|}{} \\
\hline
Goal-Cond E2E BC&0.70&	0.83&	0.70&	0.70&	0.73&	0.66&	0.74&	0.63&	0.63&	0.72\\
Goal-Cond E2E DAgger&0.61&0.79&0.66&0.63&0.49&0.64&0.80&0.64&0.43&0.45\\
\hline
 \textbf{Ablations} & \multicolumn{10}{c|}{} \\
\hline
Goal-Cond Traj. Flow&0.26&0.46&0.16&0.19&0.30&0.13&0.28&0.44&0.14&0.24\\
% {Ours w/ Lear}&0.14&0.16&0.06&0.16&0.15&0.02&0.05&0.24&0.22&0.09\\
{Goal-Cond Goal Flow}&0.14&0.16&0.06&0.16&0.15&0.02&0.05&0.24&0.22&0.09\\
\hline
 \textbf{Ours} & \multicolumn{10}{c|}{} \\
\hline
\textbf{Goal-Cond DCP + Res. Flow}&0.11&0.12&0.02&0.06&0.15&0.05&0.12&0.28&0.10&0.07\\
\hline
\end{tabular}
}
\caption{Execution Normalized L2 Distance Metric Results ($\downarrow$): Normalized L2 distances to the ground truth goal position after rollouts. The lower the better.}
\label{tab:exec-l2-dist}
\end{table*}

==> tables/exec-sr-rate-merged.tex <==
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{|lr|rl|ll|ll|ll|ll|ll|ll|ll|ll|ll|}
\hline
\rule{0pt}{2.5em}
 & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} & \multicolumn{2}{c|}{\clipart{chair}} & \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{fridge}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{washingmachine}} & \multicolumn{2}{c|}{\clipart{safe}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-22} 
 & \multicolumn{1}{l|}{} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Baselines}}} & E2E BC & 0.02 & 0.01 & 0.03 & 0.00 & 0.10 & 0.05 & 0.03 & 0.05 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
\multicolumn{1}{|l|}{} & E2E DAgger & 0.03 & 0.00 & 0.00 & 0.00 & 0.10 & 0.00 & 0.10 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.03 & 0.00 & 0.00 & 0.00 \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Ablations}}} & Traj. Flow & 0.15 & 0.13 & 0.03 & 0.03 & 0.63 & 0.60 & 0.13 & 0.13 & 0.03 & 0.00 & 0.25 & 0.25 & 0.10 & 0.00 & 0.00 & 0.00 & 0.05 & 0.00 & 0.15 & 0.15 \\
\multicolumn{1}{|l|}{} & Goal Flow & 0.64 & 0.05 & 0.73 & 0.00 & 0.75 & 0.10 & 0.73 & 0.00 & 0.50 & 0.00 & 0.80 & 0.00 & \textbf{0.65} & 0.10 & 0.35 & 0.10 & 0.70 & 0.10 & 0.55 & 0.05 \\ \hline
\multicolumn{1}{|l|}{\textbf{Ours}} & \textbf{ACRONYM} & \textbf{0.78} & \textbf{0.81} & \textbf{0.78} & \textbf{0.78} & \textbf{0.98} & \textbf{1.00} & \textbf{0.88} & \textbf{1.00} & \textbf{0.70} & \textbf{0.73} & \textbf{1.00} & \textbf{1.00} & 0.65 & \textbf{0.65} & \textbf{0.55} & \textbf{0.45} & \textbf{0.73} & \textbf{0.88} & \textbf{0.80} & \textbf{0.80} \\ \hline
\end{tabular}
}
\caption{Execution Success Rate Metric Results ($\uparrow$): Fraction of success trials (normalized L2 distance less than 0.1 \textbf{and} there is no collision in the entire rollout trajectory) of different objects' categories after rollouts. The higher the better.}
\label{tab:exec-sr}
\end{table*}

==> tables/exec-sr-rate.tex <==
\begin{table*}[ht]
\renewcommand{\arraystretch}{1.2}
% \resizebox{\textwidth}{!}{
\centering
\resizebox{0.6\textwidth}{!}{
\setlength\tabcolsep{.2em}
\begin{tabular}{|r|c|ccccccccc|}
 \hline
 \rule{0pt}{2.5em}
 & \textbf{\underline{AVG.}} &\clipart{microwave} &\clipart{chair}&\clipart{dishwasher}&\clipart{oven}&\clipart{fridge}&\clipart{table}&\clipart{washingmachine}&\clipart{safe}&\clipart{drawer}\\
\hline
 \textbf{Baselines} & \multicolumn{10}{c|}{} \\
\hline
Goal-Cond E2E BC&0.02&	0.03&	0.10&	0.03&	0.00&	0.00&	0.00&	0.00&	0.00&	0.00\\
Goal-Cond E2E DAgger&0.03&0.00&0.10&0.10&0.00&0.00&0.00&0.00&0.03&0.00\\
\hline
 \textbf{Ablations} & \multicolumn{10}{c|}{} \\
\hline
Goal-Cond Traj. Flow&0.15&0.025&0.63&0.13&0.03&0.25&0.10&0.00&0.05&0.15\\
{Goal-Cond Goal Flow}&0.60&0.63&0.73&0.73&0.48&0.85&0.65&0.37&0.48&0.50\\
% \textbf{Ours 2/ FCL Collision Checker}&0.68&0.78&0.77&0.75&0.55&0.93&0.75&0.35&0.70&0.55\\
\hline
 \textbf{Ours} & \multicolumn{10}{c|}{} \\
\hline
\textbf{Goal-Cond DCP + Res. Flow}&0.78&0.78&0.98&0.88&0.70&1.00&0.65&0.55&0.73&0.80\\
\hline
\end{tabular}
}
\caption{Execution Success Rate Metric Results ($\uparrow$): Fraction of success trials (normalized L2 distance less than 0.1 \textbf{and} there is no collision in the entire rollout trajectory) of different objects' categories after rollouts. The higher the better.}
\label{tab:exec-sr}
\end{table*}

==> tables/gi-Rt-error.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table}[]
% \centering
% \renewcommand{\arraystretch}{1.2}
% \resizebox{\textwidth}{!}{
% \setlength\tabcolsep{.2em}
% \begin{tabular}{|lr|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|}
% \hline
%  \rule{0pt}{2.5em}
%  & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} & \multicolumn{2}{c|}{\clipart{chair}} & \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{fridge}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{washingmachine}} & \multicolumn{2}{c|}{\clipart{safe}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-22} 
%  & \multicolumn{1}{l|}{} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} \\ \hline
% \multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Baselines}}} & E2E BC & 40.45 & 0.75 & 37.82 & 0.82 & 38.17 & 0.81 & 37.15 & 0.65 & 44.84 & 0.68 & 32.52 & 1.06 & 40.38 & 0.69 & 45.09 & 0.76 & 45.00 & 0.79 & 45.65 & 0.64 \\
% \multicolumn{1}{|l|}{} & E2E DAgger & 36.85 & 0.71 & 34.15 & 0.76 & 36.50 & 0.74 & 36.61 & 0.66 & 40.91 & 0.65 & 30.67 & 0.97 & 35.95 & 0.70 & 40.34 & 0.74 & 32.86 & 0.79 & 39.45 & 0.53 \\ \hline
% \multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Ablations}}} & Traj. Flow & 35.37 & 0.66 & 31.24 & 0.82 & 33.89 & 0.69 & 39.21 & 0.72 & 34.35 & 0.66 & 28.48 & 0.75 & 37.14 & 0.59 & 29.49 & 0.70 & 39.60 & 0.76 & 39.69 & 0.48 \\
% \multicolumn{1}{|l|}{} & Goal Flow & 26.46 & 0.16 & 25.88 & 0.15 & 26.29 & 0.10 & 25.05 & 0.15 & 30.62 & 0.15 & 27.61 & 0.10 & 28.01 & 0.18 & 20.96 & 0.24 & 29.02 & 0.23 & 22.13 & 0.20 \\
% % \multicolumn{1}{|l|}{} & CPE Only & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ \hline
% \hline
% \multicolumn{1}{|l|}{\textbf{Ours}} & \textbf{TAX-Pose} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ \hline
% \end{tabular}
% }
% \caption{Goal Inference Rotational and Translational Error Results. Rotational errors ($\mathcal{E}_\mathbf{R}$) are in degrees ($^\circ$) and translational errors ($\mathcal{E}_\mathbf{t}$) are in meters ($\mathrm{m}$). }
% \label{tab:gi-Rt}
% \end{table}
% \vspace{-25pt}

% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
\begin{table}[h]
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{
\setlength\tabcolsep{.2em}
\begin{tabular}{|lr|cc|cc|cc|cc|cc|cc|cc|cc|cc|}
\hline
 \rule{0pt}{2.5em}
 & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} &  \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{fridge}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{washingmachine}} & \multicolumn{2}{c|}{\clipart{safe}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-20} 
 & \multicolumn{1}{l|}{} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Baselines}}} & E2E BC & 42.26 & 0.73 & 37.82 & 0.82 & 37.15 & 0.65 & 44.84 & 0.68 & 30.69 & 1.06 & 40.38 & 0.69 & 45.09 & 0.76 & 45.00 & 0.79 & 45.65 & 0.64 \\
\multicolumn{1}{|l|}{} & E2E DAgger~\cite{ross2011reduction} & 37.96 & 0.69 & 34.15 & 0.76 & 36.61 & 0.66 & 40.91 & 0.65 & 24.87 & 0.97 & 35.95 & 0.70 & 40.34 & 0.74 & 32.86 & 0.79 & 39.45 & 0.53 \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Ablations}}} & Traj. Flow~\cite{EisnerZhang2022FLOW} & 35.95 & 0.67 & 31.24 & 0.82 & 39.21 & 0.72 & 34.35 & 0.66 & 28.48 & 0.75 & 37.14 & 0.59 & 29.49 & 0.70 & 39.60 & 0.76 & 39.69 & 0.48 \\
\multicolumn{1}{|l|}{} & Goal Flow~\cite{EisnerZhang2022FLOW} & 26.64 & 0.17 & 25.88 & \textbf{0.15} & 25.05 & 0.15 & 30.62 & 0.15 & 27.61 & 0.10 & 28.01 & \textbf{0.18} & 20.96 & \textbf{0.24} & 29.02 & 0.23 & 22.13 & 0.20  \\
% \multicolumn{1}{|l|}{} & CPE Only & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ \hline
\hline
\multicolumn{1}{|l|}{\textbf{Ours}} & \textbf{TAX-Pose} & \textbf{6.64} & \textbf{0.16} & \textbf{6.85} & 0.16 & \textbf{2.05} & \textbf{0.10} & \textbf{3.87} & \textbf{0.12} & \textbf{4.04} & \textbf{0.08} & \textbf{12.71} & 0.31 & \textbf{6.87} & 0.37 & \textbf{5.89} & \textbf{0.13} & \textbf{14.93} & \textbf{0.18} \\ \hline
\end{tabular}
}
\caption{Goal Inference Rotational and Translational Error Results ($\downarrow$). Rotational errors ($\mathcal{E}_\mathbf{R}$) are in degrees ($^\circ$) and translational errors ($\mathcal{E}_\mathbf{t}$) are in meters ($\mathrm{m}$). The lower the better.}
\label{tab:gi-Rt}
\end{table}
% \vspace{-25pt}

==> tables/gi-chamfer-dist-merged.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|lr|rl|ll|ll|ll|ll|ll|ll|ll|ll|ll|}
\hline
 \rule{0pt}{2.5em}
 & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} & \multicolumn{2}{c|}{\clipart{chair}} & \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{fridge}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{washingmachine}} & \multicolumn{2}{c|}{\clipart{safe}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-22} 
 & \multicolumn{1}{l|}{} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{\scriptsize Baselines}}} &  E2E BC & 0.69 & 0.81 & 0.77 & 0.81 & 0.71 & 0.88 & 0.72 & 0.86 & 0.65 & 0.79 & 0.70 & 0.68 & 0.65 & 0.69 & 0.64 & 0.69 & 0.68 & 0.79 & 0.67 & 0.88 \\
\multicolumn{1}{|l|}{} &  E2E DAgger & 0.49 & 0.68 & 0.71 & 0.79 & 0.39 & 0.69 & 0.56 & 0.60 & 0.43 & 0.60 & 0.55 & 0.91 & 0.42 & 0.84 & 0.42 & 0.67 & 0.50 & 0.63 & 0.43 & 0.58 \\ \hline
\multicolumn{1}{|l|}{\multirow{4}{*}{\textbf{\scriptsize Ablations}}} &  Traj. Flow & 0.25 & 0.49 & 0.39 & 0.54 & 0.19 & 0.42 & 0.28 & 0.53 & 0.27 & 0.53 & 0.11 & 0.62 & 0.26 & 0.32 & 0.27 & 0.42 & 0.33 & 0.58 & 0.18 & 0.45 \\
\multicolumn{1}{|l|}{} &  Goal Flow & 0.14 & 0.37 & 0.10 & 0.36 & 0.06 & 0.35 & 0.16 & 0.52 & \textbf{0.15} & 0.25 & 0.07 & 0.34 & 0.05 & 0.40 & 0.24 & 0.45 & 0.22 & 0.50 & 0.18 & 0.13 \\
\multicolumn{1}{|l|}{} &  Pose Match & 0.54 & 0.53 & 0.66 & 0.66 & 0.47 & 0.48 & 0.70 & 0.69 & 0.28 & 0.29 & 0.45 & 0.43 & 0.78 & 0.73 & 0.32 & 0.33 & 0.67 & 0.68 & 0.50 & 0.44 \\
\multicolumn{1}{|l|}{} &  Pose Match WS & 0.37 & 0.36 & 0.56 & 0.54 & 0.19 & 0.18 & 0.57 & 0.53 & 0.35 & 0.28 & 0.23 & 0.18 & 0.56 & 0.33 & 0.28 & 0.41 & 0.48 & 0.54 & 0.12 & 0.22 \\ \hline
\multicolumn{1}{|l|}{\textbf{\scriptsize Ours}} &  \textbf{ACRONYM} & \textbf{0.07} & \textbf{0.08} & \textbf{0.05} & \textbf{0.08} & \textbf{0.00} & \textbf{0.02} & \textbf{0.09} & \textbf{0.05} & 0.19 & \textbf{0.21 }& \textbf{0.01} & \textbf{0.02} & \textbf{0.03} &\textbf{ 0.11} & \textbf{0.14} & \textbf{0.14} &\textbf{ 0.05} & \textbf{0.08 }& \textbf{0.08} & \textbf{0.03} \\ \hline
\end{tabular}
}
\caption{Goal Inference Normalized Chamfer Distance Metric Results ($\downarrow$): Normalized Chamfer distances to the point cloud under ground truth goal pose. The lower the better.}
\label{tab:gi-chamfer-dist}
\end{table*}

==> tables/gi-chamfer-dist.tex <==
\begin{table*}[ht]
\renewcommand{\arraystretch}{1.2}
\centering
\resizebox{0.6\textwidth}{!}{
\setlength\tabcolsep{.2em}
\begin{tabular}{|r|c|ccccccccc|}
 \hline
 \rule{0pt}{2.5em}
 & \textbf{\underline{AVG.}} &\clipart{microwave} &\clipart{chair}&\clipart{dishwasher}&\clipart{oven}&\clipart{fridge}&\clipart{table}&\clipart{washingmachine}&\clipart{safe}&\clipart{drawer}\\
\hline
 \textbf{Baselines} & \multicolumn{10}{c|}{} \\
\hline
Goal-Cond E2E BC&0.69&	0.77&	0.71&	0.72&	0.65&	0.70&	0.65&	0.64&	0.68&	0.67\\
Goal-Cond E2E DAgger&0.49&0.71&0.39&0.56&0.43&0.55&0.42&0.42&0.50&0.43\\
\hline
 \textbf{Ablations} & \multicolumn{10}{c|}{} \\
\hline
Goal-Cond Traj. Flow&0.25&0.39&0.19&0.28&0.27&0.11&0.26&0.27&0.33&0.18\\
Goal-Cond Goal Flow&0.14&0.10&0.06&0.16&0.15&0.07&0.05&0.24&0.22&0.18\\
Goal-Cond DCP&0.54&0.66&0.47&0.70&0.28&0.45&0.78&0.32&0.67&0.50\\
Goal-Cond DCP Weighted Sum&0.37	&0.56&	0.19&	0.57&	0.35&	0.23&	0.56&	0.28&	0.48&	0.12\\
\hline
 \textbf{Ours} & \multicolumn{10}{c|}{} \\
\hline
\textbf{Goal-Cond DCP + Res. Flow}&0.07&0.05&0.00&0.09&0.19&0.01&0.03&0.14&0.05&0.08\\
\hline
\end{tabular}
}
\caption{Goal Inference Normalized Chamfer Distance Metric Results ($\downarrow$): Normalized Chamfer distances to the point cloud under ground truth goal pose. The lower the better.}
\label{tab:gi-chamfer-dist}
\end{table*}

==> tables/gi-sr-rate-merged.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|lr|rl|ll|ll|ll|ll|ll|ll|ll|ll|ll|}
\hline
 \rule{0pt}{2.5em}
 & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} & \multicolumn{2}{c|}{\clipart{chair}} & \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{fridge}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{washingmachine}} & \multicolumn{2}{c|}{\clipart{safe}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-22} 
 & \multicolumn{1}{l|}{} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{\scriptsize Baselines}}} &  E2E BC & 0.09 & 0.03 & 0.00 & 0.00 & 0.10 & 0.00 & 0.00 & 0.05 & 0.15 & 0.00 & 0.25 & 0.00 & 0.15 & 0.10 & 0.00 & 0.10 & 0.10 & 0.00 & 0.05 & 0.00 \\
\multicolumn{1}{|l|}{} &  E2E DAgger & 0.31 & 0.05 & 0.00 & 0.30 & 0.50 & 0.03 & 0.23 & 0.03 & 0.33 & 0.03 & 0.50 & 0.00 & 0.25 & 0.00 & 0.15 & 0.10 & 0.40 & 0.00 & 0.40 & 0.00 \\ \hline
\multicolumn{1}{|l|}{\multirow{4}{*}{\textbf{\scriptsize Ablations}}} &  Traj. Flow & 0.61 & 0.39 & 0.28 & 0.13 & 0.75 & 0.50 & 0.53 & 0.50 & 0.50 & 0.15 & 0.80 & 0.75 & 0.80 & 0.20 & 0.55 & 0.50 & 0.50 & 0.25 & 0.75 & 0.50 \\
\multicolumn{1}{|l|}{} &  Goal Flow & 0.74 & 0.42 & 0.75 & 0.40 & 0.88 & 0.63 & 0.78 & 0.22 & \textbf{0.80} & 0.60 & 0.83 & 0.50 & 0.75 & 0.50 & 0.65 & 0.05 & 0.63 & 0.25 & 0.65 & 0.65 \\
\multicolumn{1}{|l|}{} &  Pose Match & 0.29 & 0.30 & 0.25 & 0.20 & 0.30 & 0.30 & 0.00 & 0.00 & 0.68 & 0.58 & 0.38 & 0.43 & 0.10 & 0.00 & 0.45 & 0.65 & 0.10 & 0.18 & 0.40 & 0.40 \\
\multicolumn{1}{|l|}{} &  Pose Match WS & 0.38 & 0.44 & 0.20 & 0.20 & 0.65 & 0.63 & 0.05 & 0.15 & 0.45 & 0.60 & 0.58 & 0.38 & 0.15 & 0.50 & 0.45 & 0.35 & 0.28 & 0.20 & 0.65 & 0.65 \\ \hline
\multicolumn{1}{|l|}{\textbf{\scriptsize Ours}} &  \textbf{ACRONYM} & \textbf{0.90} & \textbf{0.88} & \textbf{0.93} & \textbf{0.88} & \textbf{1.00} & \textbf{0.98} & \textbf{0.85} & \textbf{0.95} & 0.80 & \textbf{0.70} & \textbf{1.00} & \textbf{1.00 }& \textbf{0.95} & \textbf{0.80} & \textbf{0.75} & \textbf{0.75} & \textbf{0.95 }& \textbf{0.93 }& \textbf{0.90} & \textbf{0.95} \\ \hline
\end{tabular}
}
\caption{Goal Inference Success Rate Metric Results ($\uparrow$): Fraction of success trials (normalized Chamfer distance less than 0.1) of different objects' categories in goal inference only. The higher the better.}
\label{tab:gi-sr}
\end{table*}

==> tables/gi-sr-rate.tex <==
\begin{table*}[ht]
\renewcommand{\arraystretch}{1.2}
\centering
\resizebox{0.6\textwidth}{!}{
\setlength\tabcolsep{.2em}
\begin{tabular}{|r|c|ccccccccc|}
 \hline
 \rule{0pt}{2.5em}
 & \textbf{\underline{AVG.}} &\clipart{microwave} &\clipart{chair}&\clipart{dishwasher}&\clipart{oven}&\clipart{fridge}&\clipart{table}&\clipart{washingmachine}&\clipart{safe}&\clipart{drawer}\\
\hline
 \textbf{Baselines} & \multicolumn{10}{c|}{} \\
\hline
Goal-Cond E2E BC&0.09&	0.00&	0.10&	0.00&	0.15&	0.25&	0.15&	0.00&	0.10&	0.05\\
Goal-Cond E2E DAgger&0.31&0.00&0.50&0.23&0.33&0.50&0.25&0.15&0.40&0.40\\
\hline
 \textbf{Ablations} & \multicolumn{10}{c|}{} \\
\hline
Goal-Cond Traj. Flow&0.61&0.28&0.75&0.53&0.50&0.80&0.80&0.55&0.50&0.75\\
{Goal-Cond Goal Flow}&0.74&0.75&0.88&0.78&0.80&0.83&0.75&0.65&0.625&0.65\\
Goal-Cond DCP&0.29&0.25&0.30&0.00&0.68&0.38&0.10&0.45&0.10&0.40\\
Goal-Cond DCP Weighted Sum&0.38&	0.20&	0.65&	0.05&	0.45&	0.58&	0.15&	0.45&	0.275&	0.65\\
\hline
 \textbf{Ours} & \multicolumn{10}{c|}{} \\
\hline
\textbf{Goal-Cond DCP + Res. Flow}&0.90&0.93&1.00&0.85&0.80&1.00&0.95&0.75&0.95&0.90\\
\hline
\end{tabular}
}
\caption{Goal Inference Success Rate Metric Results ($\uparrow$): Fraction of success trials (normalized Chamfer distance less than 0.1) of different objects' categories in goal inference only. The higher the better.}
\label{tab:gi-sr}
\end{table*}

==> tables/gi_sim_Rt_goal0.tex <==
\begin{table}[H]
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{
\setlength\tabcolsep{.2em}
\begin{tabular}{|lr|cc|cc|cc|cc|cc|cc|cc|cc|cc|}
\hline
 \rule{0pt}{2.5em}
 & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} &  \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{fridge}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{washingmachine}} & \multicolumn{2}{c|}{\clipart{safe}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-20} 
 & \multicolumn{1}{l|}{} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Baselines}}} & E2E BC & 42.37 & 0.69 & 40.49 & 0.80 & 50.79 & 0.59 & 48.02 & 0.61 & 30.69 & 1.09 & 36.59 & 0.81 & 48.48 & 0.42 & 41.42 & 0.84 & 42.49 & 0.37 \\
\multicolumn{1}{|l|}{} & E2E DAgger~\cite{ross2011reduction} & 36.06 & 0.67 & 38.57 & 0.68 & 43.99 & 0.63 & 42.34 & 0.57 & 24.87 & 0.96 & 30.87 & 0.90 & 42.96 & 0.46 & 29.79 & 0.83 & 35.08 & 0.33 \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Ablations}}} & Traj. Flow~\cite{EisnerZhang2022FLOW} & 34.48 & 0.65 & 35.39 & 0.85 & 43.42 & 0.63 & 35.51 & 0.60 & 28.26 & 0.80 & 27.67 & 0.68 & 25.91 & 0.44 & 43.59 & 0.82 & 36.05 & 0.36 \\
\multicolumn{1}{|l|}{} & Goal Flow~\cite{EisnerZhang2022FLOW} & 27.49 & \textbf{0.21} & 25.41 & \textbf{0.08} & 31.07 & 0.13 & 27.05 & 0.27 & 27.80 & 0.11 & 29.02 & \textbf{0.38} & 19.22 & \textbf{0.36} & 31.56 & 0.18 & \textbf{28.81} & \textbf{0.19} \\
% \multicolumn{1}{|l|}{} & CPE Only & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ \hline
\hline
\multicolumn{1}{|l|}{\textbf{Ours}} & \textbf{TAX-Pose} & \textbf{11.74} & 0.23 & {\textbf{5.81}} & {0.11} & {\textbf{1.82}} & {\textbf{0.08}} & {\textbf{5.92}} & {\textbf{0.11}} & {\textbf{3.67}} & {\textbf{0.07}} & {\textbf{19.54}} & {0.41} & {\textbf{7.96}} & {0.63} & {\textbf{5.96}} & {\textbf{0.12}} & {43.27} & {0.33} \\ \hline
\end{tabular}
}
\caption{Goal Inference Rotational and Translational Error Results ($\downarrow$) for the ``\textbf{In'}' Goal. Rotational errors ($\mathcal{E}_\mathbf{R}$) are in degrees ($^\circ$) and translational errors ($\mathcal{E}_\mathbf{t}$) are in meters ($\mathrm{m}$). The lower the better.}
\label{tab:gi-Rt_goal0}
\end{table}

==> tables/gi_sim_Rt_goal1.tex <==
\begin{table}[H]
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{
\setlength\tabcolsep{.2em}
\begin{tabular}{|lr|cc|cc|cc|cc|cc|cc|cc|}
\hline
 \rule{0pt}{2.5em}
 & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} &  \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{washingmachine}} & \multicolumn{2}{c|}{\clipart{safe}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-16} 
 & \multicolumn{1}{l|}{} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Baselines}}} & E2E BC & 42.69 & 0.74 & 41.94 & 0.74 & 36.70 & 0.52 & 38.23 & 0.73 & 41.69 & 1.10 & 48.57 & 0.75 & 48.98 & 0.63 \\
\multicolumn{1}{|l|}{} & E2E DAgger~\cite{ross2011reduction} & 37.68 & 0.70 & 39.24 & 0.69 & 31.63 & 0.54 & 41.06 & 0.68 & 37.72 & 1.03 & 35.94 & 0.75 & 40.47 & 0.51 \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Ablations}}} & Traj. Flow~\cite{EisnerZhang2022FLOW} & 35.13 & 0.76 & 34.78 & 0.70 & 39.14 & 0.59 & 31.10 & 0.69 & 33.07 & 0.97 & 35.61 & 0.71 & 37.09 & 0.87 \\
\multicolumn{1}{|l|}{} & Goal Flow~\cite{EisnerZhang2022FLOW} & 22.10 & 0.20 & 27.82 & 0.26 & 20.43 & \textbf{0.09} & 34.66 & 0.10 & 22.71 & 0.12 & 26.48 & 0.27 & 0.48 & 0.32 \\
% \multicolumn{1}{|l|}{} & CPE Only & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ \hline
\hline
\multicolumn{1}{|l|}{\textbf{Ours}} & \textbf{TAX-Pose} & \textbf{4.45} & \textbf{0.12} & \textbf{4.21} & \textbf{0.12} & \textbf{2.29} & 0.10 & \textbf{2.73} & \textbf{0.09} & \textbf{5.77} & \textbf{0.10} & \textbf{5.81} & \textbf{0.13} & \textbf{5.89} & \textbf{0.19} \\ \hline
\end{tabular}
}
\caption{Goal Inference Rotational and Translational Error Results ($\downarrow$) for the ``\textbf{On}'' Goal. Rotational errors ($\mathcal{E}_\mathbf{R}$) are in degrees ($^\circ$) and translational errors ($\mathcal{E}_\mathbf{t}$) are in meters ($\mathrm{m}$). The lower the better.}
\label{tab:gi-Rt_goal1}
\end{table}

==> tables/gi_sim_Rt_goal2.tex <==
\begin{table}[H]
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{
\setlength\tabcolsep{.2em}
\begin{tabular}{|lr|cc|cc|cc|cc|cc|cc|cc|}
\hline
 \rule{0pt}{2.5em}
 & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} &  \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{fridge}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-16} 
 & \multicolumn{1}{l|}{} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Baselines}}} & E2E BC & 44.87 & 0.74 & 30.95 & 0.89 & 36.86 & 0.72 & 56.86 & 0.52 & 34.35 & 1.03 & 31.69 & 0.77 & 46.86 & 0.78 \\
\multicolumn{1}{|l|}{} & E2E DAgger~\cite{ross2011reduction} & 41.32 & 0.68 & 31.40 & 0.84 & 38.49 & 0.73 & 47.64 & 0.51 & 36.47 & 0.99 & 27.72 & 0.73 & 39.83 & 0.51 \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Ablations}}} & Traj. Flow~\cite{EisnerZhang2022FLOW} & 38.85 & 0.58 & 31.87 & 1.07 & 39.48 & 0.44 & 39.48 & 0.44 & 28.71 & 0.69 & 41.06 & 0.73 & 40.70 & 0.31 \\
\multicolumn{1}{|l|}{} & Goal Flow~\cite{EisnerZhang2022FLOW} & 29.64 & \textbf{0.10} & 28.51 & \textbf{0.10} & 26.33 & \textbf{0.08} & 32.96 & \textbf{0.07} & 27.42 & 0.10 & 22.04 & \textbf{0.09} & 27.42 & 0.15  \\
% \multicolumn{1}{|l|}{} & CPE Only & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ \hline
\hline
\multicolumn{1}{|l|}{\textbf{Ours}} & \textbf{TAX-Pose} & \textbf{6.02} & 0.17 & \textbf{12.73} & 0.28 & \textbf{1.59} & 0.11 & \textbf{2.91} & 0.12 & \textbf{4.41} & \textbf{0.08} & \textbf{12.12} & 0.34 & \textbf{6.38} & \textbf{0.12} \\ \hline
\end{tabular}
}
\caption{Goal Inference Rotational and Translational Error Results ($\downarrow$) for the ``\textbf{Left}'' Goal. Rotational errors ($\mathcal{E}_\mathbf{R}$) are in degrees ($^\circ$) and translational errors ($\mathcal{E}_\mathbf{t}$) are in meters ($\mathrm{m}$). The lower the better.}
\label{tab:gi-Rt_goal2}
\end{table}

==> tables/gi_sim_Rt_goal3.tex <==
\begin{table}[H]
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{
\setlength\tabcolsep{.2em}
\begin{tabular}{|lr|cc|cc|cc|cc|cc|cc|}
\hline
 \rule{0pt}{2.5em}
 & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} &  \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-14} 
 & \multicolumn{1}{l|}{} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Baselines}}} & E2E BC & 39.11 & 0.76 & 37.89 & 0.86 & 24.26 & 0.77 & 36.27 & 0.88 & 52.86 & 0.48 & 44.26 & 0.78 \\
\multicolumn{1}{|l|}{} & E2E DAgger~\cite{ross2011reduction} & 36.80 & 0.73 & 27.40 & 0.84 & 32.31 & 0.74 & 32.61 & 0.82 & 49.27 & 0.46 & 42.40 & 0.78 \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Ablations}}} & Traj. Flow~\cite{EisnerZhang2022FLOW} & 35.33 & 0.71 & 22.93 & 0.66 & 34.78 & 1.22 & 31.29 & 0.92 & 42.71 & 0.37 & 44.93 & 0.36 \\
\multicolumn{1}{|l|}{} & Goal Flow~\cite{EisnerZhang2022FLOW} & 27.34 & 0.16 & 21.79 & 0.15 & 22.37 & 0.28 & 27.79 & 0.15 & 32.96 & \textbf{0.07} & 31.79 & 0.15  \\
% \multicolumn{1}{|l|}{} & CPE Only & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ \hline
\hline
\multicolumn{1}{|l|}{\textbf{Ours}} & \textbf{TAX-Pose} & \textbf{4.33} & \textbf{0.13} & \textbf{4.64} & \textbf{0.14} & \textbf{2.48} & \textbf{0.11} & \textbf{3.91} & \textbf{0.15} & \textbf{6.47} & 0.17 & \textbf{4.17} & \textbf{0.08} \\ \hline
\end{tabular}
}
\caption{Goal Inference Rotational and Translational Error Results ($\downarrow$) for the ``\textbf{Right}'' Goal. Rotational errors ($\mathcal{E}_\mathbf{R}$) are in degrees ($^\circ$) and translational errors ($\mathcal{E}_\mathbf{t}$) are in meters ($\mathrm{m}$). The lower the better.}
\label{tab:gi-Rt_goal3}
\end{table}

==> tables/mug_on_rack_exp.tex <==
\begin{table}[h]
    % \small
    \centering
    \begin{tabular}{c|c c c| c c c}
    \hline
     & \textbf{Grasp} & \textbf{Place} & \textbf{Overall} & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
    % & Grasp & Place & Overall\\
    \hline
    %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 1^{\circ}$}}\\
     &\multicolumn{3}{c}{\textbf{Upright Pose}}& \multicolumn{3}{c}{\textbf{Arbitrary Pose}} \\
         \hline
         DON \cite{florence2018dense} & 0.91 &0.50 & 0.45 & 0.35 & 0.45& 0.17 \\
         NDF \cite{simeonov2021neural} &  0.96 & 0.92 & 0.88  & \textbf{0.78} &0.75 & 0.58\\
         \textbf{TAX-Pose (Ours)} & \textbf{0.99}& \textbf{0.97}& \textbf{0.96} &  0.75& \textbf{0.84}& \textbf{0.63}\\
         
    \hline
        %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 5^{\circ}$}}\\

    % \textbf{Arbitrary Pose} & & & \\
    %  \hline
    %      DON \cite{florence2018dense} & 0.35 & 0.45& 0.17 \\
    %      NDF \cite{simeonov2021neural} & \textbf{0.78} &0.75 & 0.58\\
    %       TAX-Pose (Ours)  &  0.75& \textbf{0.84}& \textbf{0.63}\\
         
    % \hline
    \end{tabular}
    \caption{Mug on Rack Simulation Task Success Results
    % \dave{Let's make this table horizontal to save space (put ``arbitrary pose" to the right of upright pose) - OR wrap text around it}
    }
    \label{tab:mug_on_rack_exp}
\end{table}
% \vspace{-1em}
% \begin{table}[h]
%     \centering
%     \begin{tabular}{c|c c c}
%     \hline
%      & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
%     % & Grasp & Place & Overall\\
%     \hline
%     %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 1^{\circ}$}}\\
%     \hline
%         \textbf{Upright Pose} & & &\\
%          \hline
%          DON \cite{florence2018dense} & 0.91 &0.50 & 0.45\\
%          NDF \cite{simeonov2021neural} &  0.96 & 0.92 & 0.88 \\
%          TAX-Pose (Ours) & \textbf{0.99}& \textbf{0.97}& \textbf{0.96}\\
         
%     \hline
%         %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 5^{\circ}$}}\\

%     \textbf{Arbitrary Pose} & & & \\
%      \hline
%          DON \cite{florence2018dense} & 0.35 & 0.45& 0.17 \\
%          NDF \cite{simeonov2021neural} & \textbf{0.78} &0.75 & 0.58\\
%           TAX-Pose (Ours)  &  0.75& \textbf{0.84}& \textbf{0.63}\\
         
%     \hline
%     \end{tabular}
%     \caption{Mug on Rack Simulation Task Success Results
%     \dave{Let's make this table horizontal to save space (put ``arbitrary pose" to the right of upright pose) - OR wrap text around it}
%     }
 
%     \label{tab:mug_on_rack_exp}
% \end{table}

==> tables/mug_on_rack_few_shot.tex <==
% \begin{table}[h]
% \begin{subtable}[h]{0.1\textwidth}
%     \centering
%       \begin{adjustbox}{0.2\textwidth}
%     \begin{tabular}{c|c c c}
%     % \hline
%      \textbf{Model} & \multicolumn{3}{c} \#\textbf{Demos Used }\\
%     \hline
%           & 1 & 5 & 10\\
%          \hline
%          DON \cite{florence2018dense}  & 0.32 &0.36 & 0.45\\
%          NDF \cite{simeonov2021neural} &  0.46 & 0.70 & 0.88 \\
%           TAX-Pose (Ours) & \textbf{0.77}& \textbf{0.90}& \textbf{0.96}\\
         
%     \hline
 
    
%     \end{tabular}
%         \end{adjustbox}
%     %\caption{Mug on Rack Simulation Task Success Results with Varying Number of Demo Used
%     %\dave{Too much whitespace around this table; wrap text around it}
%     %}
 
%     %  \label{tab:mug_on_rack_few_shot}
     
%  \end{subtable}

% % \hfill
% \begin{subtable}[h]{0.1\textwidth}
%     \centering
%      \begin{adjustbox}{0.2\textwidth}
%     \begin{tabular}{c|c c c}
%     \hline
%     \textbf{Ablation} & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
  
%     %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 1^{\circ}$}}\\
   
%         % \textbf{Upright Pose} & & &\\
%          \hline
%          No Residual Correspondence  & 0.97 &0.96 & 0.93\\
%          Unweighted SVD &  0.92 & 0.94 & 0.88 \\
%          3-Layer MLP In Place of Attention &  0.90 & 0.82 & 0.76 \\
%          TAX-Pose (Ours)  & \textbf{0.99}& \textbf{0.97}& \textbf{0.96}\\
         
%     \hline
     
%     \end{tabular}
%     \end{adjustbox}

 
%   #%\label{tab:mug_rack_ablation}
%  \end{subtable}
%     \caption{Mug on Rack Ablation  Results}
%     \label{tab:mug_rack_ablation}
% \end{table}


%  \begin{table}[h]
 
%     \centering
     
%     \begin{tabular}{c|c c c}
%     % \hline
%      \textbf{Model} & \multicolumn{3}{c} \#\textbf{Demos Used }\\
%     \hline
%           & 1 & 5 & 10\\
%          \hline
%          DON \cite{florence2018dense}  & 0.32 &0.36 & 0.45\\
%          NDF \cite{simeonov2021neural} &  0.46 & 0.70 & 0.88 \\
%           TAX-Pose (Ours) & \textbf{0.77}& \textbf{0.90}& \textbf{0.96}\\
         
%     \hline
 
    
%     \end{tabular}
        
%     \caption{Analysis of Number of Demonstrations Used in Training on Upright Pose Mug Hanging Task Success
%     % \dave{Too much whitespace around this table; wrap text around it}
%     }
 
%      \label{tab:mug_on_rack_few_shot}
     
%  \end{table}


% \begin{table}[h]
% \begin{varwidth}[b]{0.33\linewidth}
%     \centering
%     \begin{tabular}{c|c c c}
%     \textbf{Model} & \multicolumn{3}{c} \#\textbf{Demos Used }\\
%     \hline
%           & 1 & 5 & 10\\
%          \hline
%          DON \cite{florence2018dense}  & 0.32 &0.36 & 0.45\\
%          NDF \cite{simeonov2021neural} &  0.46 & 0.70 & 0.88 \\
%           TAX-Pose (Ours) & \textbf{0.77}& \textbf{0.90}& \textbf{0.96}\\
%     \hline
%     \end{tabular}
%     \caption{Analysis of Number of Demonstrations Used in Training on Upright Pose Mug Hanging Task Success}
%      \label{tab:mug_on_rack_few_shot}
% \end{varwidth}%
% \begin{varwidth}[b]{0.2\linewidth}
%     \centering
%     \begin{tabular}{c|c c c}
%     \hline
%     \textbf{Ablation} & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
  
%     %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 1^{\circ}$}}\\
   
%         % \textbf{Upright Pose} & & &\\
%          \hline
%          No Residual Correspondence  & 0.97 &0.96 & 0.93\\
%          Unweighted SVD &  0.92 & 0.94 & 0.88 \\
%          3-Layer MLP In Place of Attention &  0.90 & 0.82 & 0.76 \\
%          TAX-Pose (Ours)  & \textbf{0.99}& \textbf{0.97}& \textbf{0.96}\\
         
%     \hline
%     \end{tabular}
%     \caption{Mug Hanging Ablations Results}
%     \label{tab:mug_rack_ablation}
% \end{varwidth}%

% \end{table}

 
 \begin{wraptable}{r}{8cm}
 
    \centering
     
    \begin{tabular}{c|c c c}
    % \hline
     \textbf{Model} & \multicolumn{3}{c} \#\textbf{Demos Used }\\
    \hline
          & 1 & 5 & 10\\
         \hline
         DON \cite{florence2018dense}  & 0.32 &0.36 & 0.45\\
         NDF \cite{simeonov2021neural} &  0.46 & 0.70 & 0.88 \\
          TAX-Pose (Ours) & \textbf{0.77}& \textbf{0.90}& \textbf{0.96}\\
         
    \hline
 
    
    \end{tabular}
        
    \caption{Analysis of Number of Demonstrations Used in Training on Upright Pose Mug Hanging Task Success
    % \dave{Too much whitespace around this table; wrap text around it}
    }
 
     \label{tab:mug_on_rack_few_shot}
     
 \end{wraptable}
 

==> tables/mug_rack_ablation.tex <==
% \begin{table}[h]
\begin{table}[]
  \tiny
    \centering
    \begin{tabular}{c|c c c}
    \hline
    \textbf{Ablation} & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
  
    %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 1^{\circ}$}}\\
   
        % \textbf{Upright Pose} & & &\\
         \hline
         No Residual Correspondence  & 0.97 &0.96 & 0.93\\
         Unweighted SVD &  0.92 & 0.94 & 0.88 \\
         3-Layer MLP In Place of Attention &  0.90 & 0.82 & 0.76 \\
         TAX-Pose (Ours)  & \textbf{0.99}& \textbf{0.97}& \textbf{0.96}\\
         
    \hline
    \end{tabular}
    \caption{Mug Hanging Ablations Results}
    \label{tab:mug_rack_ablation}
\end{table}



 

==> tables/mug_rack_ablation_large_scale.tex <==
% % \begin{table}[h]
% \begin{table}[H]
 
%     \centering
% \renewcommand{\arraystretch}{1.2}
% \resizebox{\textwidth}{!}{
%     \begin{tabular}{c|c| c c c}
%     \hline
%   \textbf{Ablation Category} & \textbf{Ablation Experiment} & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
  
%     %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 1^{\circ}$}}\\
   
%         % \textbf{Upright Pose} & & &\\
%          \hline
     
%          \multirow{4}{*}{\textit{Loss}}  & No $\mathcal{L}_\mathrm{disp}$ &  0.01 & 0 & 0 \\
%          & No $ \mathcal{L}_\mathrm{corr}$ &  0.89 & 0.91 & 0.84 \\
%          & No $  \mathcal{L}_\mathrm{cons}$ &  \textbf{0.99} & 0.95 & 0.94 \\
%          & Scaled Combination of  $ \mathcal{L}_\mathrm{corr} \&   \mathcal{L}_\mathrm{cons}$ ($ 1.1*\mathcal{L}_\mathrm{cons} + 1*\mathcal{L}_\mathrm{corr}$) &  0.10 & 0.01 & 0.01 \\
%          \hline 
%          \multirow{1}{*}{\textit{Residual Correspondence}}  & No Residual Correspondence  & 0.97 &0.96 & 0.93\\
         
%          \hline 
%          \multirow{1}{*}{\textit{Weighted SVD}} & 
%          Unweighted SVD &  0.92 & 0.94 & 0.88 \\
         
%         \hline 
%         \multirow{2}{*}{\textit{Pretraining Embedding Network}} &
     
%          No Finetuning for Embedding Network &  0.98 & 0.93 & 0.91 \\
%          & No Pretraining for Embedding Network &  \textbf{0.99} & 0.72 & 0.71 \\
         
%          \hline 
%         \multirow{1}{*}{\textit{Architecture for Cross-Object Attention}} & 
%          3-Layer MLP In Place of Transformer &  0.90 & 0.82 & 0.76 \\
         
         
%         \hline
%       \multirow{1}{*}{\textit{\# Dimensions for Embedding}} &
%         Embedding Network Feature Dim = 16 & 0.98 & 0.59 & 0.57 \\
    
%         \hline
%         \hline
%         \textbf{\textit{Ours}} & \textbf{TAX-Pose}  & \textbf{0.99}& \textbf{0.97}& \textbf{0.96}\\

         
%     \hline
%     \end{tabular}
%     }
%     \caption{Mug Hanging Ablations Results Full Scale}
%     \label{tab:mug_rack_ablation_full}
% \end{table}



 % \begin{table}[h]
\begin{table}[H]
 
    \centering
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{
    \begin{tabular}{c| c c c}
    \hline
  \textbf{Ablation Experiment} & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
  
    %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 1^{\circ}$}}\\
   
        % \textbf{Upright Pose} & & &\\
         \hline
        \textit{Loss}&&&\\
          No $\mathcal{L}_\mathrm{disp}$ &  0.01 & 0 & 0 \\
          No $ \mathcal{L}_\mathrm{corr}$ &  0.89 & 0.91 & 0.84 \\
           No $  \mathcal{L}_\mathrm{cons}$ &  \textbf{0.99} & 0.95 & 0.94 \\
            Scaled Combination of  $ \mathcal{L}_\mathrm{corr} \&   \mathcal{L}_\mathrm{cons}$ ($ (1.1)\mathcal{L}_\mathrm{cons} + \mathcal{L}_\mathrm{corr}$) &  0.10 & 0.01 & 0.01 \\
         \hline 
          No Adjustment via Correspondence Residuals  & 0.97 &0.96 & 0.93\\
         \hline 
         Unweighted SVD &  0.92 & 0.94 & 0.88 \\
        \hline 
         No Finetuning for Embedding Network &  0.98 & 0.93 & 0.91 \\
         No Pretraining for Embedding Network &  \textbf{0.99} & 0.72 & 0.71 \\
         \hline 
         3-Layer MLP In Place of Transformer &  0.90 & 0.82 & 0.76 \\
        \hline
        Embedding Network Feature Dim = 16 & 0.98 & 0.59 & 0.57 \\
    
        \hline
        \hline
        \textbf{TAX-Pose (Ours)}  & \textbf{0.99}& \textbf{0.97}& \textbf{0.96}\\

         
    \hline
    \end{tabular}
    }
    \caption{Mug Hanging Ablations Results}
    \label{tab:mug_rack_ablation_full}
\end{table}



 

==> tables/nauc_100_50.tex <==
\begin{table}[b]
    \centering
    \begin{tabular}{c|c c c}
    \hline
    Algorithm & Mean nAUC & Max nAUC & Min nAUC \\
    \hline
        %  PRC &              12.78 & 36.11 & 5.42 \\
         $SO(3)$ &  27.00 & 86.43 & 9.80 \\
         $SO(3)$ w/ PMG~\cite{chen2021projective} & 16.89 & 54.00 & \textbf{4.08} \\
         Quaternion  & 25.57 & 87.95 & 4.83 \\
         MRP (Ours) & \textbf{7.29} & \textbf{17.94} & 4.35\\
    \hline
    \end{tabular}
    \caption{Normalized Area Under Curve (nAUC) of global angular error over 50 unique environments with 100 randomly generated orientations each. Maximum of 300K optimization steps.}
    %in $SO(3)$.} 
    % each. , run over 50 sets of orientation sets each with 100 randomly generated orientations in $SO(3)$}
    \label{tab:AUC_N100_S50}
\end{table}

==> tables/nauc_50_200.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{c|c c c}
    \hline
    Algorithm & Mean nAUC & Max nAUC & Min nAUC \\
    \hline
        %  PRC &              3.37 & 11.98 & 1.36\\
         $SO(3)$ &  5.79 & 23.29 & 2.78\\
         $SO(3)$ \w PMG \cite{chen2021projective} & 3.66 & 25.40 & 0.90 \\
         Quaternion & 4.24 & 81.24 & 0.91 \\
         PRC & \textbf{1.69} & \textbf{4.91} & \textbf{0.98}\\
         
    \hline
    \end{tabular}
    \caption{Normalized Area Under Curve (nAUC) of global angular error for 50 orientations, run over 200 sets of orientation sets each with 50 randomly generated orientations in $SO(3)$}
    \label{tab:AUC_N50_S200}
\end{table}


==> tables/nauc_50_50.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{c|c c c}
    \hline
    Algorithm & Mean nAUC & Max nAUC & Min nAUC \\
    \hline
         PRC &  3.19 &  6.29 &  1.68\\
         $SO(3)$ Log Map& 5.64& 15.04 & 2.78\\
         $SO(3)$ PMG \cite{chen2021projective} & 4.02& 13.27&1.12\\
         Quat Cosine & 5.27& 81.24&1.08\\
         PRC-BP & 1.73 &3.55 & 1.09\\
    \hline
    \end{tabular}
    \caption{Normalized Area Under Curve (nAUC) of global angular error for 50 orientations, run over 50 sets of orientation sets each with 50 randomly generated orientations in $SO(3)$}
    \label{tab:AUC_N50_S50}
\end{table}

==> tables/percent_converged_100_50.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{c|c c c c c c c c}
    \hline
        & \multicolumn{5}{c}{\textit{\% Avg Pairwise Angular Error $ < 5^{\circ}$}}\\
    Algorithm & 30K  & 70K  & 100K  & 150K  & 300K \\
    \hline
    % & \multicolumn{5}{c}{\textit{\% Avg Pairwise Angular Error $ < 1^{\circ}$}}\\
    % \hline
    %     %  PRC &12  & 74 & 90 & 100 &  100\\
    %      $SO(3)$ &  0 & 0 & 0 & 6 &  88\\
    %      $SO(3)$ w/ PMG~\cite{chen2021projective} & 0 & 12 & 34 & 56 &  82 \\
    %      Quaternion &  0 & 8 & 18 & 40 & 70\\
    %      MRP (Ours) & \textbf{60} & \textbf{86}  & \textbf{96} & \textbf{98}  & \textbf{100}  \\
    % \hline
    \hline
        %  PRC & 28  & 82 & 92 & 100 &  100\\
         $SO(3)$ &  0\% & 0\% & 12\% & 66\% &  96\%\\
         $SO(3)$ w/ PMG~\cite{chen2021projective} & 4\% & 34\% & 52\% & 72\% &  92\% \\
         Quaternion &  2\% & 22\% & 38\% & 58\% & 82\% \\
         MRP (Ours) & \textbf{76}\% & \textbf{88}\%  & \textbf{96}\% & \textbf{98}\%  & \textbf{100}\%  \\
    \hline
    \end{tabular}
    \caption{Percentage of experiments converged over 50 unique environments with 100 randomly generated orientations each. We take 300K optimization steps for each experiment.}
    %  100 orientations, run over 50 sets of orientation sets each with 50 randomly generated orientations in $SO(3)$}
    \label{tab:percent_converge_N100_S50}
\end{table}

% \begin{table}[h]
%     \centering
%     \begin{tabular}{c|c c c c c c c c}
%     \hline
%     Algorithm & 30K & 70K & 100K & 150K & 300K \\
%     \hline
%          PRC & 0.12  & 0.74 & 0.9 & 1 &  1\\
%          $SO(3)$ Log Map&  0 & 0 & 0 & 0.06 &  0.88\\
%          $SO(3)$ PMG \cite{chen2021projective} & 0 & 0.12 & 0.34 & 0.56 &  0.82 \\
%          Quat Cosine &  0 & 0.08 & 0.18 & 0.4 & 0.7\\
%          PRC-BP &  &   &  &   &   \\
%     \hline
%     \end{tabular}
%     \caption{Percentage of experiments converged within 100 orientations, run over 50 sets of orientation sets each with 50 randomly generated orientations in $SO(3)$}
%     \label{tab:percent_converge_N100_S50}
% \end{table}

==> tables/percent_converged_50_200.tex <==
% \begin{table}[h]
%     \centering
%     \begin{tabular}{c|c c c c c}
%     \hline
%     Algorithm & 5K & 10K & 20K & 40K & 150K \\
%     \hline
%          PRC &  0.20 & 0.84 & 0.99 & 1 & 1\\
%          $SO(3)$ Log Map&  0 & 0 & 0.19 & 0.98  &  1\\
%          $SO(3)$ PMG \cite{chen2021projective} & 0.05 & 0.42 & 0.81 & 0.95  & 1 \\
%          Quat Cosine &  0.03 & 0.33 & 0.75 & 0.95 &  0.99\\
%          PRC-BP &   &   &   &  &      \\
%     \hline
%     \end{tabular}
%     \caption{Percentage of experiments converged within 50 orientations, run over 200 sets of orientation sets each with 50 randomly generated orientations in $SO(3)$}
%     \label{tab:percent_converge_N5
%     0_S200}
% \end{table}



\begin{table}[h]
    \centering
    \begin{tabular}{c|c c c c c}
    \hline
    Algorithm & 5K& 10K& 20K & 40K & 150K\\
    \hline
    & \multicolumn{5}{c}{\textit{\% Avg Pairwise Angular Error $ < 1^{\circ}$}}\\
    \hline
         PRC &  20 &84 & 99 & 100 & 100\\
         $SO(3)$ Log Map&  0 & 0 & 19 & 98  &  100\\
         $SO(3)$ PMG \cite{chen2021projective} & 5 & 42 & 81 & 95  & 100 \\
         Quat Cosine &  3 & 34 & 76 & 95 &  99\\
         PRC-BP &  89 & 99  & 100  & 100 &    100  \\
    \hline
    & \multicolumn{5}{c}{\textit{\% Avg Pairwise Angular Error $ < 5^{\circ}$}}\\
    \hline
         PRC &  39 & 90 &100 & 100 & 100\\
         $SO(3)$ Log Map&  0 & 0.5 & 85.5 & 99 &  100\\
         $SO(3)$ PMG \cite{chen2021projective} & 16.5 & 63.5 & 91.0 & 98.5  & 100 \\
         Quat Cosine &  19.5 & 59.5 & 88 & 97 &  99\\
         PRC-BP & 92  & 98  &  100 & 100 & 100     \\
    \hline
    \end{tabular}
    \caption{Percentage of experiments converged within 50 orientations, run over 200 sets of orientation sets each with 50 randomly generated orientations in $SO(3)$}
    \label{tab:percent_converge_N50_S200}
\end{table}

==> tables/percent_converged_50_50.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{c|c c c c c c c c}
    \hline
    Algorithm & 5K & 10K & 20K & 40K & 150K\\
    \hline
        & \multicolumn{5}{c}{\textit{\% Avg Pairwise Angular Error $ < 1^{\circ}$}}\\
    \hline
         PRC &  22  & 86  & 100 & 100  &  100\\
         $SO(3)$ Log Map&  0 & 0 & 20 & 100&  100\\
         $SO(3)$ PMG \cite{chen2021projective} & 6 &30 & 76  & 92 & 100 \\
         Quat Cosine &  0 & 32 & 74 & 92 & 98\\
         PRC-BP &  90& 98 & 100  & 100  & 100  \\
    \hline
        & \multicolumn{5}{c}{\textit{\% Avg Pairwise Angular Error $ < 5^{\circ}$}}\\
    \hline
         PRC &  42  & 92  & 100 & 100  &  100\\
         $SO(3)$ Log Map&  0 & 0 & 84 & 100&  100\\
         $SO(3)$ PMG \cite{chen2021projective} & 10 &56 & 88  & 100 & 100 \\
         Quat Cosine &  16 & 58 & 90 & 94 & 98\\
         PRC-BP &  92 & 98 & 100  & 100  & 100  \\
    \hline
    \end{tabular}
    \caption{Percentage of experiments converged within 50 orientations, run over 50 sets of orientation sets each with 50 randomly generated orientations in $SO(3)$}
    \label{tab:percent_converge_N50_S50}
\end{table}

==> tables/rw-placement.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
% \centering
% \begin{tabular}{|r|c|c|c|c|}
% \hline
% \multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{\textbf{AVG. SR}} & \multicolumn{1}{l|}{\clipart{drawer}} & \multicolumn{1}{l|}{\clipart{fridge}} & \multicolumn{1}{l|}{\clipart{oven}} \\ \hline
% Goal Flow & 0.31 & 0.18 & 0.38 & 0.37 \\ \hline
% \textbf{TAX-Pose} & 0.92 & 0.95 & 0.95 & 0.85 \\ \hline
% \end{tabular}
\begin{tabular}{|r|c|c|c|}
\hline
\multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{\clipart{drawer}} & \multicolumn{1}{l|}{\clipart{fridge}} & \multicolumn{1}{l|}{\clipart{oven}} \\ \hline
Goal Flow & 0.18 & 0.38 & 0.37 \\ \hline
\textbf{TAX-Pose} & 0.95 & 0.95 & 0.85 \\ \hline
\end{tabular}
\label{rw-placement}
\caption{PartNet-Mobility Objects Placement Task Real-World Results.}
\end{table}

==> tables/rw_each.tex <==
\begin{table}[H]
\renewcommand{\arraystretch}{1.2}
\resizebox{0.6\textwidth}{!}{
\setlength\tabcolsep{.2em}
\begin{tabular}{|l|lll|lll|lll|}
\hline
\multirow{2}{*}{} & \multicolumn{3}{c|}{\textbf{In}} & \multicolumn{3}{c|}{\textbf{On}} & \multicolumn{3}{c|}{\textbf{Left}} \\ \cline{2-10} 
 & \multicolumn{1}{l|}{\clipart{drawer}} & \multicolumn{1}{l|}{\clipart{fridge}} & \clipart{oven} & \multicolumn{1}{l|}{\clipart{drawer}} & \multicolumn{1}{l|}{\clipart{fridge}} & \clipart{oven} & \multicolumn{1}{l|}{\clipart{drawer}} & \multicolumn{1}{l|}{\clipart{fridge}} & \clipart{oven} \\ \hline
Goal Flow & \multicolumn{1}{l|}{0.00} & \multicolumn{1}{l|}{0.10} & 0.30 & \multicolumn{1}{l|}{0.05} & \multicolumn{1}{l|}{N/A} & 0.20 & \multicolumn{1}{l|}{0.50} & \multicolumn{1}{l|}{0.65} & 0.60 \\
\textbf{TAX-Pose} & \multicolumn{1}{l|}{\textbf{1.00}} & \multicolumn{1}{l|}{\textbf{1.00}} & \textbf{0.85} & \multicolumn{1}{l|}{\textbf{1.00}} & \multicolumn{1}{l|}{N/A} & \textbf{1.00} & \multicolumn{1}{l|}{\textbf{0.85}} & \multicolumn{1}{l|}{\textbf{0.90}} & \textbf{0.70} \\ \hline
\end{tabular}
}
\caption{Combined per-task results for real-world goal placement success rate.}
\label{tab:rw_each}
\end{table}

==> tables/single_goal.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[h]
\begin{subtable}[h]{\textwidth}
    \centering
    \begin{tabular}{|lr|rl|ll|ll|ll|ll|ll|ll|ll|ll|ll|}
    \hline
    \rule{0pt}{2.5em}
    
    & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} & \multicolumn{2}{c|}{\clipart{chair}} & \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{fridge}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{washingmachine}} & \multicolumn{2}{c|}{\clipart{safe}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-22} 
    
    & \multicolumn{1}{l|}{} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} \\ \hline
    
    \end{tabular}
    \caption{First Week}
    \label{tab:week1}
\end{subtable}
\begin{subtable}[h]{\textwidth}
        \centering
        \begin{tabular}{l | l | l}
        Day & Max Temp & Min Temp \\
        \hline \hline
        Mon & 20 & 13\\
        Tue & 22 & 14\\
        Wed & 23 & 12\\
        Thurs & 25 & 13\\
        Fri & 18 & 7\\
        Sat & 15 & 13\\
        Sun & 20 & 13
       \end{tabular}
      \caption{First Week}
       \label{tab:week2}
\end{subtable}
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{|lr|rl|ll|ll|ll|ll|ll|ll|ll|ll|ll|}
% \hline
%  \rule{0pt}{2.5em}
%  & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} & \multicolumn{2}{c|}{\clipart{chair}} & \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{fridge}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{washingmachine}} & \multicolumn{2}{c|}{\clipart{safe}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-22} 
%  & \multicolumn{1}{l|}{} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} \\ \hline
% \multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{\scriptsize Baselines}}} &  E2E BC & 0.69 & 0.81 & 0.77 & 0.81 & 0.71 & 0.88 & 0.72 & 0.86 & 0.65 & 0.79 & 0.70 & 0.68 & 0.65 & 0.69 & 0.64 & 0.69 & 0.68 & 0.79 & 0.67 & 0.88 \\
% \multicolumn{1}{|l|}{} &  E2E DAgger & 0.49 & 0.68 & 0.71 & 0.79 & 0.39 & 0.69 & 0.56 & 0.60 & 0.43 & 0.60 & 0.55 & 0.91 & 0.42 & 0.84 & 0.42 & 0.67 & 0.50 & 0.63 & 0.43 & 0.58 \\ \hline
% \multicolumn{1}{|l|}{\multirow{4}{*}{\textbf{\scriptsize Ablations}}} &  Traj. Flow & 0.25 & 0.49 & 0.39 & 0.54 & 0.19 & 0.42 & 0.28 & 0.53 & 0.27 & 0.53 & 0.11 & 0.62 & 0.26 & 0.32 & 0.27 & 0.42 & 0.33 & 0.58 & 0.18 & 0.45 \\
% \multicolumn{1}{|l|}{} &  Goal Flow & 0.14 & 0.37 & 0.10 & 0.36 & 0.06 & 0.35 & 0.16 & 0.52 & \textbf{0.15} & 0.25 & 0.07 & 0.34 & 0.05 & 0.40 & 0.24 & 0.45 & 0.22 & 0.50 & 0.18 & 0.13 \\
% \multicolumn{1}{|l|}{} &  Pose Match & 0.54 & 0.53 & 0.66 & 0.66 & 0.47 & 0.48 & 0.70 & 0.69 & 0.28 & 0.29 & 0.45 & 0.43 & 0.78 & 0.73 & 0.32 & 0.33 & 0.67 & 0.68 & 0.50 & 0.44 \\
% \multicolumn{1}{|l|}{} &  Pose Match WS & 0.37 & 0.36 & 0.56 & 0.54 & 0.19 & 0.18 & 0.57 & 0.53 & 0.35 & 0.28 & 0.23 & 0.18 & 0.56 & 0.33 & 0.28 & 0.41 & 0.48 & 0.54 & 0.12 & 0.22 \\ \hline
% \multicolumn{1}{|l|}{\textbf{\scriptsize Ours}} &  \textbf{ACRONYM} & \textbf{0.07} & \textbf{0.08} & \textbf{0.05} & \textbf{0.08} & \textbf{0.00} & \textbf{0.02} & \textbf{0.09} & \textbf{0.05} & 0.19 & \textbf{0.21 }& \textbf{0.01} & \textbf{0.02} & \textbf{0.03} &\textbf{ 0.11} & \textbf{0.14} & \textbf{0.14} &\textbf{ 0.05} & \textbf{0.08 }& \textbf{0.08} & \textbf{0.03} \\ \hline
% \end{tabular}
% }
\caption{Ben testing something o}
\label{tab:single-goal}
\end{table}

==> tables/steps_converge_100_50.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{c|c c c}
    \hline
     & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 5^{\circ}$}}\\
     Algorithm & Mean Steps & Max Steps & Min Steps\\
    \hline
    %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 1^{\circ}$}}\\
    % \hline
    %     %  PRC &  57.20 & 140.00 & 20.00  \\
    %      $SO(3)$ &  216.1K & Not Converged & 140.0K \\
    %      $SO(3)$ w/ PMG~\cite{chen2021projective} & 163.2K & Not Converged & 36.0K \\
    %      Quaternion & 196.8K & Not Converged & 50.0K  \\
    %      MRP (Ours) & \textbf{39.2K}  & \textbf{175.0K}  & \textbf{15.0K} \\
    % \hline
    \hline
        %  PRC &  50.40 & 135.00 & 15.00  \\
         $SO(3)$ &  153.0K & Not Converged & 80.0K \\
         $SO(3)$ w/ PMG~\cite{chen2021projective} & 120.7K & Not Converged & 21.0K \\
         Quaternion & 152.1K & Not Converged & 30.0K  \\
         MRP (Ours) &  \textbf{32.5K} & \textbf{155.0K}  & \textbf{10.0K} \\
    \hline
    \end{tabular}
    \caption{Number of iteration steps until convergence over 50 unique environments with 100 randomly generated orientations each. We take 300K optimization steps for each experiment.}
    %within 100 orientations, run over 50 sets of orientation sets each with 100 randomly generated orientations in $SO(3)$, after 300K optimization steps.}
    \label{tab:steps_converge_N100_S50}
\end{table}

==> tables/steps_converge_50_200.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{c|c c c}
    \hline
    Algorithm & Mean Steps(K) & Max Steps(K) & Min Steps(K)\\
    \hline
    & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $ < 1^{\circ}$}}\\
    \hline
         PRC &  7.74 & 28.00 & 3.5  \\
         $SO(3)$ Log Map&  24.10 & 58.00 & 16.50 \\
         $SO(3)$ PMG \cite{chen2021projective} & 15.44 & 77.50 & 4.00 \\
         Quat Cosine & 766.42 & does not converge & 4.50  \\
         PRC-BP &   &   &  \\
    \hline
    & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $ < 5^{\circ}$}}\\
    \hline
         PRC &  6.64 & 27.00 & 2.50  \\
         $SO(3)$ Log Map&  16.70 & 52.00 & 10.00 \\
         $SO(3)$ PMG \cite{chen2021projective} & 10.80 & 49.50 & 2.50 \\
         Quat Cosine & 12.91 & does not converge & 2.0  \\
         PRC-BP &   &   &  \\
    \hline
    \end{tabular}
    \caption{Iteration steps till convergence within 50 orientations, run over 200 sets of orientation sets each with 200 randomly generated orientations in $SO(3)$, after 150K optimization steps.}
    \label{tab:steps_converge_N50_S200}
\end{table}

% \begin{table}[h]
%     \centering
%     \begin{tabular}{c|c c c}
%     \hline
%     Algorithm & Mean Steps (K) & Max Steps (K) & Min Steps (K)\\
%     \hline
%          PRC &  7742 & 28000 & 3500  \\
%          $SO(3)$ Log Map&  24105 & 58000 & 16500 \\
%          $SO(3)$ PMG \cite{chen2021projective} & 15445 & 77500 & 4000 \\
%          Quat Cosine & 766427 & 150000 (DN) & 4500  \\
%          PRC-BP &   &   &  \\
%     \hline
%     \end{tabular}
%     \caption{Iteration steps till convergence within 50 orientations, run over 50 sets of orientation sets each with 200 randomly generated orientations in $SO(3)$, ones labeled with \textbf{DN} means does not converge within 300K steps}
%     \label{tab:steps_converge_N50_S200}
% \end{table}

==> tables/steps_converge_50_50.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{c|c c c}
    \hline
    Algorithm & Mean Steps(K) & Max Steps(K) & Min Steps(K)\\
    \hline
    & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $ < 1^{\circ}$}}\\
    \hline
         PRC &  7.44 & 13.50 & 4.00  \\
         $SO(3)$ Log Map&  23.67 & 38.00 & 17.00 \\
         $SO(3)$ PMG \cite{chen2021projective} & 17.30 & 69.50 & 4.50 \\
         Quat Cosine & 20.73 & does not converge & 5.50  \\
         PRC-BP & 3.88  &13.00   &2.00  \\
    \hline
        & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $ < 5^{\circ}$}}\\
    \hline
         PRC &  6.34 & 12.50 & 3.00  \\
         $SO(3)$ Log Map&  16.44 & 31.50 & 10.50 \\
         $SO(3)$ PMG \cite{chen2021projective} & 12.04 & 37.50 & 3.00 \\
         Quat Cosine & 15.23 & does not converge & 3.50  \\
         PRC-BP & 3.46  & 12.50  & 2.00 \\
    \hline
    \end{tabular}
        \caption{Iteration steps till convergence within 50 orientations, run over 50 sets of orientation sets each with 50 randomly generated orientations in $SO(3)$, after 150K optimization steps.}
    % \caption{Iteration steps till convergence within 50 orientations, run over 50 sets of orientation sets each with 50 randomly generated orientations in $SO(3)$, ones labeled with \textbf{DN} means does not converge within 300K steps}
    \label{tab:steps_converge_N50_S50}
\end{table}

% \begin{table}[h]
%     \centering
%     \begin{tabular}{c|c c c}
%     \hline
%     Algorithm & Mean & Max & Min \\
%     \hline
%          PRC &  7440 & 13500 & 4000  \\
%          $SO(3)$ Log Map&  23670 & 38000 & 17000 \\
%          $SO(3)$ PMG \cite{chen2021projective} & 17300 & 69500 & 4500 \\
%          Quat Cosine & 20730 & 150000 (DN) & 5500  \\
%          PRC-BP &   &   &  \\
%     \hline
%     \end{tabular}
%     \caption{Iteration steps till convergence within 50 orientations, run over 50 sets of orientation sets each with 50 randomly generated orientations in $SO(3)$, ones labeled with \textbf{DN} means does not converge within 300K steps}
%     \label{tab:steps_converge_N50_S50}
% \end{table}
